Anthropomorphic Twisted String-Actuated Soft Robotic Gripper with Tendon-Based Stiffening

Realizing high-performance soft robotic grippers is challenging because of the inherent limitations of the soft actuators and artificial muscles that drive them, including low force output, small actuation range, and poor compactness. Despite advances in this area, realizing compact soft grippers with high dexterity and force output is still challenging. This paper explores twisted string actuators (TSAs) to drive a soft robotic gripper. TSAs have been used in numerous robotic applications, but their inclusion in soft robots has been limited. The proposed design of the gripper was inspired by the human hand. Tunable stiffness was implemented in the fingers with antagonistic TSAs. The fingers' bending angles, actuation speed, blocked force output, and stiffness tuning were experimentally characterized. The gripper achieved a score of 6 on the Kapandji test and recreated 31 of the 33 grasps of the Feix GRASP taxonomy. It exhibited a maximum grasping force of 72 N, which was almost 13 times its own weight. A comparison study revealed that the proposed gripper exhibited equivalent or superior performance compared to other similar soft grippers.

==> ComparisonTable.tex <==
\begin{table}[]
\centering
\caption{Comparison Table}
\label{tab:comparison_table}
\begin{tabular}{|c|c|c|c|c|}
\hline
{\textbf{Soft Gripper}}     & 
\begin{tabular}{@{}c@{}}\textbf{Actuators} \\ \textbf{Used}\end{tabular}&
{ \textbf{DOFs}} & 
\begin{tabular}{@{}c@{}}\textbf{Kapandji} \\ \textbf{Test Scores}\end{tabular}&
\begin{tabular}{@{}c@{}}\textbf{GRASP} \\ \textbf{Grasps}\end{tabular}\\ \hline
%
\begin{tabular}{@{}c@{}}RBO Hand \\ 2 \cite{Deimal2016}\end{tabular} 
& \begin{tabular}{@{}c@{}}Pneumatic \\ Actuators\end{tabular} 
& 7 & 9 & 31 \\ \hline
%
\begin{tabular}{@{}c@{}}BCL--13 \\ \cite{Jianshu2018}\end{tabular} 
& \begin{tabular}{@{}c@{}}Pneumatic \\ Actuators\end{tabular} 
& 13 & 8 & -- \\ \hline
%
\begin{tabular}{@{}c@{}}BCL--26 \\ \cite{Jianshu2019}\end{tabular} 
& \begin{tabular}{@{}c@{}}Pneumatic \\ Actuators\end{tabular} 
& 26 & 10 & 33 \\ \hline
%
\begin{tabular}{@{}c@{}}RBO Hand \\ 3 \cite{RBO3}\end{tabular} 
& \begin{tabular}{@{}c@{}}Pneumatic \\ Actuators\end{tabular} 
&16 & 10 & 33 \\ \hline
%
Our Gripper 
& TSAs & 6 & 6 & 31 \\ \hline
%
\end{tabular}
\end{table}

==> figures/2.tex <==
\begin{comment}
\begin{figure}
    \centering
    \subfloat[]{
    \includegraphics[height=6cm]{images/fig1b.png}}
    \hfill
    \subfloat[]{
    \includegraphics[height=6cm]{images/fig1.jpg}}
    \hfill
    \caption{(a) Schematic of the twisted string actuator (TSA). (b) Photograph of the assembled robotic hand.}
    \label{fig:2}
\end{figure}
\end{comment}

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{images/tsa_sorting_mechanism.png}
    \caption{\textcolor{red}{Schematic of the TSA with the fixed twisting zone and sorter mechanism.}}
    \label{fig:tsa_sorting_mechanism}
\end{figure}

==> figures/KapandjiTest.tex <==
\begin{figure}
    \centering
    \includegraphics[height=6cm]{images/KapandjiTest/KapandjiSummary.PNG}
    \caption{The Kapandji Test gives a measure of thumb dexterity by counting the number of points on the hand the tip of the thumb can touch. Attainable contacts are shown in green and failed locations are shown in red.}
    \label{fig:KapandjiTest}
\end{figure}

==> figures/basediagram.tex <==
\begin{figure}
    \centering
    \includegraphics[height=5cm]{images/design/BaseDrawing4.PNG}
    \hfill
    \caption{Computer-drafted model of base with major components labeled.}
    \label{fig:basediagram}
\end{figure}

==> figures/fullgripperCAD.tex <==
\begin{figure}
    \centering
    \includegraphics[height=6cm]{images/design/Full4.PNG}
    \caption{Computer-drafted model of the full gripper. All dimensions shown are in mm.}
    \label{fig:fullgripperCAD}
\end{figure}

==> figures/poses.tex <==
\begin{figure*}
    \centering
    \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/poses/index_thum.PNG}}
    \hfill
    %
    \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/poses/middle_thumb.PNG}}
    %
    \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/poses/ring_thumb.PNG}}
    \hfill
    %
    \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/poses/pinky_thumb.PNG}}
    \hfill
    %
    \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/poses/dumbell.PNG}}
    \hfill
    %
    \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/poses/ball.PNG}}
    \hfill
    %
    \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/poses/pen.PNG}}
    \hfill
    %
    \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/poses/tape.JPEG}}
    \hfill
    %
    \subfloat[]{
    \includegraphics[width=0.1\linewidth]{images/poses/key.PNG}}
    \hfill
    \caption{(a)--(d): An example of the thumb's range of motion. The thumb can individually touch the (a) index finger, (b) middle finger, (c) ring finger, and (d) little finger. (e)--(f): Power grasps. The hand holding a (e) 2-kg dumbbell and (f) a rehabilitation ball. (g)--(h): Precision grasps: The hand holding a (g) pen, and (h) a roll of electrical tape. (i) Pinch grasp: The hand holding a key.}
    \label{fig:poses}
\end{figure*}

==> figures/stiffness.tex <==
\begin{figure*}
    \centering
    \subfloat[]{
    \includegraphics[height=4.5cm]{images/stiffness_image.png}}
    \hfill
    %
    \subfloat[]{
    \includegraphics[height=4.5cm]{images/stiffness_barChart.pdf}}
    \hfill
    %
    \subfloat[]{
    \includegraphics[height=4.5cm]{images/const_angle_changing_load.pdf}}
    \hfill
    %
    \caption{(a) The location of the inertial measurement unit (IMU) and hanging load during the experiments on adjustable stiffness. The setup for (a, top) was used during the experiments measuring angular deflections at varying amount of pretwist in the primary and antagonistic TSAs. The setup for (a, bottom) was used for experiments in which the motor angle was increased to in order to compensate for the angular deflections that were induced by the increasing load.}
    \label{fig:stiffness}
\end{figure*}

==> figures/thumbdiagram.tex <==
\begin{figure}
    \centering
    \float{
    \includegraphics[height=6cm]{images/design/ThumbDrawing6.PNG}}
    \hfill
    \caption{Drawing of the thumb attachment with referenced features labeled.}
    \label{fig:thumbdiagram}
\end{figure}

==> tables/quantile_stats.tex <==
\begin{table}[]
\centering
\caption{Quantile Statistics For Each Finger}
\label{tab:quantile-stats}
\begin{tabular}{|c|c|c|c|c|}
\hline
Finger & $\delta_{0}$ & $\delta_{0.25}$ & $\delta_{0.75}$ & $\delta_{1}$ \\ \hline
Index & 15.892$^{\circ}$ & 6.815$^{\circ}$ & 5.789$^{\circ}$ & 16.648$^{\circ}$ \\ \hline
Middle & 8.129$^{\circ}$ & 3.254$^{\circ}$ & 4.917$^{\circ}$ & 12.898$^{\circ}$ \\ \hline
Ring & 16.965$^{\circ}$ & 6.253$^{\circ}$ & 5.965$^{\circ}$ & 13.574$^{\circ}$ \\ \hline
Little & 18.198$^{\circ}$ & 7.996$^{\circ}$ & 5.010$^{\circ}$ & 10.310$^{\circ}$ \\ \hline
All & 20.222$^{\circ}$ & 6.437$^{\circ}$ & 6.208$^{\circ}$ & 20.489$^{\circ}$ \\ \hline
\end{tabular}
\end{table}
